Do planets remember how they formed?

One of the most directly observable features of a transiting multi-planet system is their size-ordering when ranked in orbital separation. Kepler has revealed a rich diversity of outcomes, from perfectly ordered systems, like Kepler-80, to ostensibly disordered systems, like Kepler-20. Under the hypothesis that systems are born via preferred formation pathways, one might reasonably expect non-random size-orderings reflecting these processes. However, subsequent dynamical evolution, often chaotic and turbulent in nature, may erode this information and so here we ask - do systems remember how they formed? To address this, we devise a model to define the entropy of a planetary system's size-ordering, by first comparing differences between neighboring planets and then extending to accommodate differences across the chain. We derive closed-form solutions for many of the micro state occupancies and provide public code with look-up tables to compute entropy for up to ten-planet systems. All three proposed entropy definitions exhibit the expected property that their credible interval increases with respect to a proxy for time. We find that the observed Kepler multis display a highly significant deficit in entropy compared to a randomly generated population. Incorporating a filter for systems deemed likely to be dynamically packed, we show that this result is robust against the possibility of missing planets too. Put together, our work establishes that Kepler systems do indeed remember something of their younger years and highlights the value of information theory for exoplanetary science.

==> journals.tex <==
%\newcommand{\aj}{{\it AJ}}%
          % Astronomical Journal
\newcommand{\actaa}{{\it Acta Astron.}}%
          % Acta Astronomica
%\newcommand{\araa}{{\it ARA\&A}}%
          % Annual Review of Astron and Astrophys
%\newcommand{\apj}{{\it ApJ}}%
          % Astrophysical Journal
%\newcommand{\apjl}{{\it ApJ}}%
          % Astrophysical Journal, Letters
%\newcommand{\apjs}{{\it ApJS}}%
          % Astrophysical Journal, Supplement
%\newcommand{\ao}{{\it Appl.~Opt.}}%
          % Applied Optics
%\newcommand{\apss}{{\it Ap\&SS}}%
          % Astrophysics and Space Science
%\newcommand{\aap}{{\it A\&A}}%
          % Astronomy and Astrophysics
%\newcommand{\aapr}{{\it A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
%\newcommand{\aaps}{{\it A\&AS}}%
          % Astronomy and Astrophysics, Supplement
%\newcommand{\azh}{{\it AZh}}%
          % Astronomicheskii Zhurnal
%\newcommand{\baas}{{\it BAAS}}%
          % Bulletin of the AAS
\newcommand{\caa}{{\it Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{{\it Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
%\newcommand{\icarus}{{\it Icarus}}%
  % Icarus
\newcommand{\jcap}{{\it J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
%\newcommand{\jrasc}{{\it JRASC}}%
          % Journal of the RAS of Canada
%\newcommand{\memras}{{\it MmRAS}}%
          % Memoirs of the RAS
%\newcommand{\mnras}{{\it MNRAS}}%
          % Monthly Notices of the RAS
\newcommand{\na}{{\it New A}}%
  % New Astronomy
\newcommand{\nar}{{\it New A Rev.}}%
  % New Astronomy Review
%\newcommand{\pra}{{\it Phys.~Rev.~A}}%
          % Physical Review A: General Physics
%\newcommand{\prb}{{\it Phys.~Rev.~B}}%
          % Physical Review B: Solid State
%\newcommand{\prc}{{\it Phys.~Rev.~C}}%
          % Physical Review C
%\newcommand{\prd}{{\it Phys.~Rev.~D}}%
          % Physical Review D
%\newcommand{\pre}{{\it Phys.~Rev.~E}}%
          % Physical Review E
%\newcommand{\prl}{{\it Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand{\pasa}{{\it PASA}}%
  % Publications of the Astron. Soc. of Australia
%\newcommand{\pasp}{{\it PASP}}%
          % Publications of the ASP
%\newcommand{\pasj}{{\it PASJ}}%
          % Publications of the ASJ
%\newcommand{\qjras}{{\it QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand{\rmxaa}{{\it Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
%\newcommand{\skytel}{{\it S\&T}}%
          % Sky and Telescope
%\newcommand{\solphys}{{\it Sol.~Phys.}}%
          % Solar Physics
%\newcommand{\sovast}{{\it Soviet~Ast.}}%
          % Soviet Astronomy
%\newcommand{\ssr}{{\it Space~Sci.~Rev.}}%
          % Space Science Reviews
%\newcommand{\zap}{{\it ZAp}}%
          % Zeitschrift fuer Astrophysik
%\newcommand{\nat}{{\it Nature}}%
          % Nature
%\newcommand{\iaucirc}{{\it IAU~Circ.}}%
          % IAU Cirulars
%\newcommand{\aplett}{{\it Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
%\newcommand{\apspr}{{\it Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
%\newcommand{\bain}{{\it Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
%\newcommand{\fcp}{{\it Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
%\newcommand{\gca}{{\it Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
%\newcommand{\grl}{{\it Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
%\newcommand{\jcp}{{\it J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
%\newcommand{\jgr}{{\it J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
%\newcommand{\jqsrt}{{\it J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
%\newcommand{\memsai}{{\it Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
%\newcommand{\nphysa}{{\it Nucl.~Phys.~A}}%
          % Nuclear Physics A
%\newcommand{\physrep}{{\it Phys.~Rep.}}%
          % Physics Reports
%\newcommand{\physscr}{{\it Phys.~Scr}}%
          % Physica Scripta
%\newcommand{\planss}{{\it Planet.~Space~Sci.}}%
          % Planetary Space Science
%\newcommand{\procspie}{{\it Proc.~SPIE}}%
          % Proceedings of the SPIE
